Continual Few-Shot Learning with Adversarial Class Storage

Humans have a remarkable ability to quickly and effectively learn new concepts in a continuous manner without forgetting old knowledge. Though deep learning has made tremendous successes on various computer vision tasks, it faces challenges for achieving such human-level intelligence. In this paper, we define a new problem called continual few-shot learning, in which tasks arrive sequentially and each task is associated with a few training samples. We propose Continual Meta-Learner (CML) to solve this problem. CML integrates metric-based classification and a memory-based mechanism along with adversarial learning into a meta-learning framework, which leads to the desirable properties: 1) it can quickly and effectively learn to handle a new task; 2) it overcomes catastrophic forgetting; 3) it is model-agnostic. We conduct extensive experiments on two image datasets, MiniImageNet and CIFAR100. Experimental results show that CML delivers state-of-the-art performance in terms of classification accuracy on few-shot learning tasks without catastrophic forgetting.

==> Continual Few-Shot Learning_Arxiv/1-Abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
Humans have a remarkable ability to quickly and effectively learn new concepts in a continuous manner without forgetting old knowledge.
Though deep learning has made tremendous successes on various computer vision tasks,
it faces challenges for achieving such human-level intelligence.
In this paper, we define a new problem called continual few-shot learning,
in which tasks arrive sequentially and each task is associated with a few training samples.
We propose Continual Meta-Learner (CML) to solve this problem. 
CML integrates metric-based classification and a memory-based mechanism along with adversarial learning into a meta-learning framework,
which leads to the desirable properties:
1) it can quickly and effectively learn to handle a new task;
2) it overcomes catastrophic forgetting;
3) it is model-agnostic. We conduct extensive experiments on two image datasets, MiniImageNet and CIFAR100.
Experimental results show that CML delivers state-of-the-art performance in terms of classification accuracy on few-shot learning tasks without catastrophic forgetting.

\end{abstract} 

==> Continual Few-Shot Learning_Arxiv/2-Intro.tex <==
\section{Introduction}
\IEEEPARstart{H}{umans} have a remarkable ability to effectively and quickly learn new concepts
in a continuous manner without forgetting old knowledge.
%
Even though deep learning %~\cite{LeCun2015,Schmidhuber2015}
has made tremendous successes on various computer vision tasks,
%
%it still faces huge challenges for achieving such human-level intelligence.
%
a huge amount of labeled data are usually needed to train a deep model,
which can then be used only for a specific task (e.g., classifying several types of animals).
Moreover, it has been reported that deep models may suffer from \textit{catastrophic forgetting}~\cite{Goodfellow2013}.
%
Hence, it is essential to improve deep learning such that a deep model can learn to handle a new task
from very limited training data without forgetting old knowledge.

To tackle the few-shot learning problem~\cite{Li2006,Lake2011},
a popular framework named meta-learning~\cite{Thrun1998} 
%Schmidhuber1997
is introduced, in which
a meta-learner is required to guide a learner which can rapidly learn new concepts from a small dataset with only a few samples (e.g., 5) for each class.
Recently, a few methods~\cite{Finn2017,Snell2017,Gidaris2018}
have been proposed to solve the few-shot learning problem. Even though they can significantly reduce the amount of labeled
training data and help AI go one step closer to human-level intelligence, they may suffer from catastrophic forgetting, i.e.,
forgetting or even completely forgetting what they have already learned.

Continual learning focuses on how to achieve a good trade-off between learning new concepts and retaining old knowledge over a long time, which is known as the \textit{stability-plasticity dilemma}~\cite{Mermillod2013}.
%
Several regularization-based methods~\cite{Aljundi2018,Kirkpatrick2017,Li2018,Zenke2017} have been proposed for continual learning to alleviate catastrophic forgetting. 
%
Another approach~\cite{Draelos2017,Rusu2016} introduces additional neural resources to prevent catastrophic forgetting, but usually suffers from high complexities and high memory consumption. Moreover, none of these continual learning methods
address the issue of learning new concepts with very limited labeled data, which is a key challenge for achieving human-level AI.

% \Red{Since the abilities needed in the above problem settings are both important to develop human-level artificial intelligence, we believe the proposed continual few-shot learning setting is more realistic and can better represent the process of continuously learning new concepts of a human.} 
Although solving the above problems is extremely significant, each of them suffers one-sidedness when depicting human-level learning.
%
% We believe that continual few-shot learning, which is more realistic and can better represent the process of continuously learning new concepts of a human.}
%
In this paper, by introducing continual few-shot learning which is more realistic, we aim to bridge the gap between few-shot learning and continual learning by seeking a meta-learner, which can keep learning new concepts effectively and quickly from limited labeled data without forgetting old knowledge.
We consider a scenario, where during the meta-testing phase~\cite{Ravi2017}, new tasks arrive in a sequence rather than in a batch. In this case, a meta-learner has to learn for new tasks as regular meta-learners, and meanwhile, overcome catastrophic forgetting.

Even though an existing meta-learner (such as MAML~\cite{Finn2017}) can be slightly modified to deal with continual few-shot learning tasks,
we show via experiments that it suffers from catastrophic forgetting.
%
%Since meta-learning and continual learning both have been studied recently, the most straightforward way for continual meta-learning is to fine-tune an existing meta-learner (such as MAML\cite{Finn2017}) whenever a new task arrives. However, we show via experiments that this method cannot overcome catastrophic forgetting and it  is extremely unstable when the support dataset only has 1 or 5 samples per class.
%
A straightforward solution to continual few-shot learning is to combine an existing meta-learner (such as MAML~\cite{Finn2017}) with a continual learning
method (such as MAS~\cite{Aljundi2018}). Unfortunately, our experimental results show that it still cannot effectively overcome the forgetting problem.
%
We propose a novel model-agnostic meta-learner, Continual Meta-Learner (CML), which
integrates metric-based classification and a memory-based mechanism along with adversarial
learning into an optimization-based meta-learning framework.
%
%which consists of a pre-trained teacher network extracting features, and a student generator
%generating class representations.
%%
%The scores of each sample for each class is calculated as the cosine similarity between the feature and class representation.
%%
%CML also includes a discriminator, which is used along with adversarial training~\cite{Kurakin2016} to help the generator
%generate more discriminative representations and thus improve the accuracy.
%
% We conduct extensive experiments
Comprehensive experiments have been conducted
on two widely-used datasets, MiniImageNet~\cite{Vinyals2016} and CIFAR100~\cite{Krizhevsky2009}.
%
The extensive experimental results have shown that CML delivers the state-of-the-art performance in terms of classification accuracy on few-shot learning tasks without catastrophic forgetting; 
%
while the optimization-based meta-learning approach (such as MAML) suffers from serious forgetfulness.
%
%
%
%The rest of the paper is organized as follows: In Section~\cite{Sec:Related}, we discuss the related work. In Section~\ref{Sec:Method}, we define
%the continual meta-learning problem and present the proposed CML. We present and analyze the experimental results In Section~\ref{Sec:Results} and conclude the paper in Section~\cite{Sec:Conclusions}.

%------------------------------------------------------------------------ 

==> Continual Few-Shot Learning_Arxiv/3-Related.tex <==
%====================================================================
\begin{figure*}[!ht]
\setlength{\abovecaptionskip}{0pt}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[scale=0.6]{Figure/CML.png}
\end{center}
\caption{Inference on the $n^{th}$ task of Continual Meta-Learner (CML). The Student Network takes $\bD_{train}$ to generate the all-class matrix $\bV_n$ for current task and store them into the Class Storage Module (CSM).
The pre-trained Teacher Network extracts the feature map $\bM_t$ for each test image of tasks $\mathcal{T}_{i} (i = 1, \dots, n)$.
The Classifier retrieves the all-class matrix $\bV_i$ for previous tasks $\mathcal{T}_{i} (i = 1, \dots, n-1)$ using the
label space $\bY_i$. 
Then the prediction is finished by the Classifier given the $\bM_t$ and corresponding $\bV_i (i = 1, \dots, n)$.}
\label{Fig:CML}
\end{figure*}
%====================================================================

\section{Related Work}
%In this section, we present a review of related works on
%meta-learning and continual learning.

\subsection{Few-Shot Learning}

%Recently, more and more researchers pay attentions to meta-learning (a.k.a few-shot learning) problem since it plays an important role to achieve human-level intelligence.
%In fact, it has a long history which can be backtracked to ~\cite{Naik1992, Thrun1998}.
%The goal of meta-learning is to solve how to learn new concepts quickly given a few examples.

%Meta-learning has attracted extensive attention due to its potential of achieving human-level intelligence.
%\Red{which is the ability to quickly and effectively learn new concepts with a few examples.}.
There are a few methods exploiting similarity between samples of different classes for few-shot learning,
%
% ~\cite{Koch2015,Snell2017,Vinyals2016}
which can thus be called metric-based methods.
%Metric-based methods exploit similarity between samples of different classes for meta learning.
%
%\sout{For example,} \cite{Koch2015}
%\sout{utilized a Siamese neural network to rank similarity
%between samples.}
%\sout{based on which the class of an input image is predicted.}
%
For example,
%\sout{Vinyasl~\kETAL~}
\cite{Vinyals2016} proposed Matching Networks,
%\sout{a meta-learning model called}
which leverages the cosine similarity along with an attention mechanism for classification.
%
\cite{Snell2017} presented a model called Prototypical Networks for few-shot learning,
which is similar to Matching Networks, but leverages the Euclidean distance as the similarity metric.
%\sout{Their results showed noticeable improvements on classification accuracy.}
%
\cite{Wang2018} proposed Prototype Matching Network, which combines the benefits of Prototypical networks and Matching networks. 
%
%to mitigate the class imbalance and gain contextual embedding information.
%
% \sout{Gidaris~\kETAL~}
%\cite{Gidaris2018} tackled meta-learning tasks by developing an
%attention based few-shot classification weight generator, and redesigning the classifier of a CNN as the cosine similarity function.
%\sout{function between feature representations and classification weight vectors.}
%
Other metric-based methods have been presented in~\cite{Gidaris2018,Oreshkin2018,Qi2018,Qiao2018,Sung2018}.
%\Red{Similarly,~\cite{Qi2018} also computed the activation for new category and used cosine similarity.}
%\Red{And~\cite{Qiao2018} exploited the penultimate layer representation to generate the parameters of the last linear layer.}
%\Red{The Relation Network (RN) introduced by~\cite{Sung2018} is used to learn a distance metric which can be extended to zero-shot learning setting straightforward.}
%\Red{In~\cite{Oreshkin2018} proposed metric scaling and leveraged task conditioning learner to learn a task-dependent metric space to improve performance.}
%\Red{Their results showed noticeable improvements on classification accuracy.}
%
%Similarly, our CML also uses a similarity metric to classify images, but we train our CML in a totally different way which is similar to MAML~\cite{Finn2017} and we integrate GAN~\cite{Kurakin2016} mechanism into CML to help model finds more representative class vectors. And our CML can keep the accuracy results on every learned task rather than only on base categories.

%Related works are also successful to develop a meta-learner which is used to optimize the parameters of the learner.
Another popular approach for few-shot learning focuses on optimizing model parameters, which can thus be called
the optimization-based approach.
%
%Andrychowicz~\kETAL~\cite{Andrychowicz2016} proposed a seminal work which indicated that the design of an optimization method can be converted to a learning problem.
%
Model-Agnostic Meta-Learner (MAML)~\cite{Finn2017} is a representative optimization-based method following the meta-learning framework, which
learns a good initialization for model parameters such that the model can be quickly
updated in several gradient descent steps to handle a new task. 
% \Red{Since our CML is based on MAML, CML also follows the meta-learning framework but has a better initialization by introducing a teacher network and adversarial learning.}
% \Red{Our CML is based on MAML with a teacher network and adversarial learning to find a better initialization.}
%
%In some other works~\cite{Andrychowicz2016,Mishra2018, Ravi2017, Santoro2016}, an additional neural network is used to guide how to update the parameters of learner as the %meta-learner.
%
%\Red{In a model level,~\cite{Wang2016} did the regression over the models trained from small datasets and large datasets.}
%By introducing an unsupervised meta-training phase,~\cite{Wang2016learning} made base classes and novel classes share the same feature to gain better accuracies.
%
%\Red{From a data augmentation perspective,~\cite{Hariharan2017} applied sampled transformations to the given data to augment the data diversity.}
%
%\sout{Several other methods~}
% \cite{Andrychowicz2016,Mishra2018,Ravi2017,Santoro2016}
%\sout{utilize an additional neural network, such as LSTM, as the meta-learner.}
%
%
In a seminal work~\cite{Andrychowicz2016},
% \sout{Andrychowicz \kETAL}
the authors showed the design of an optimization algorithm can be considered as a learning problem,
and designed a LSTM-based meta-learner. 
%
%which has been shown to outperform generic and hand-designed competitors.}
%
% \sout{Ravi~\kETAL~}
\cite{Ravi2017} proposed another LSTM-based meta-learner, which generates parameters sequentially with the objective of learning a good initialization.
%
Similarly,
%\sout{Santoro~\kETAL~}
\cite{Santoro2016} proposed a meta-learner based on a memory-augmented neural network, which leverages a high-capacity external
memory for few-shot learning.
%
%In~\cite{Mishra2018}, the soft attention mechanism and temporal convolutions were combined together to build a class of meta-learners.
%
%We also train a meta-learner in CML, but use it to generate class vectors which retain class information for each task to overcome catastrophic forgetting.
%
%Even though many methods developed can learn new concepts rapidly from a few examples for each new task and have achieved tremendous successes on the meta-learning problem,
%they can only be adapted to one new task which means they will forget what they have learned from previous tasks if another new task arrives, and suffer from catastrophic %forgetting.

These related works target only at few-shot learning
without addressing continual learning or the catastrophic forgetting issue, which, however, is the main focus of this work.

\subsection{Continual Learning}

%The main goal of continual learning is to retain previous learned concepts while accommodating new concepts for a model.
Continual learning represents a long-standing challenge in the machine learning field~\cite{Hassabis2017}.
%
Several regularization-based methods 
%~\cite{Aljundi2018,Kirkpatrick2017,Li2018,Zenke2017}
have been proposed for continual learning, which impose regularization terms to restrain the update of model parameters.
%
For example,
% \sout{Li~\kETAL~}
\cite{Li2018} proposed a method called Learning without Forgetting (LwF), which uses knowledge distillation to
preserving seen knowledge.
%\sout{train the network with only new task data while preserving original capabilities.}
%
% \sout{Kirkpatrick~\kETAL~}
\cite{Kirkpatrick2017} proposed Elastic Weight Consolidation (EWC), which
uses a quadratic penalty calculated by the difference between parameters for the new task and former tasks.
%\sout{to enable continual learning.}
%
% \sout{Zenke~\kETAL~}
\cite{Zenke2017} leveraged intelligent synapses for continual learning.
%
%each of which accumulates task-relevant information over time, and exploits this information to rapidly store new memories without forgetting old ones.
%
% \sout{Aljundi~\kETAL~}
\cite{Aljundi2018} presented Memory Aware Synapses (MAS), which calculates the importance of each parameter and penalizes
the change of important parameters when learning a new task to prevent forgetting.
%
\cite{Riemer2018} proposed Meta-Experience Replay (MER), which incorporates optimization based meta-learning method into experience play. 
Particularly, though they dealt with the continual learning problem through 
meta-learning, they didn't consider the few-shot setting as we considered in this paper.
%
%They also extended the continual learning problem setting on which each task may be sampled from a variety of distributions, which is different to our continual few-shot %learning setting.}
%
%CML doesn't limit the way for training the parameters. On the contrary, it starts from the same good initialization for each new task and stores the learned knowledge into %memory after training.
%
Another widely-used approach is to leverage novel neural resources or extra memory to accommodate new concepts and retain old knowledge.
%
For exmaple,
% \sout{Rusu~\kETAL~}
\cite{Rusu2016} allocated new sub-networks for each new task while freezing the network trained from previous tasks.
%
Other works along this line include \cite{Fernando2017,Draelos2017}.
%
%Some methods~\cite{Draelos2017, Fernando2017, Zhou2012} tried to allocate the novel neural resources more dynamically.
%
%\Red{Zhou~\kETAL~\cite{Zhou2012} added additional neurons to minimize the loss and then merged existing neurons to prevent redundancy.}
%
% \sout{Fernando~\kETAL~}
%
%\cite{Fernando2017} presented PathNet, which uses agents embedded in the neural network for continual learning,
%whose task is to discover which parts of the network to re-use for new tasks.
%
% \sout{Draelos~\kETAL~}
%\cite{Draelos2017} leveraged an autoencoder for continual learning, which adds novel neural units to facilitate retaining old knowledge.
%
%Our CML also uses extra memory resource to retain old knowledge, but it stores class vectors learned from each new task into memory rather than extending and augmenting the architecture of model.
%
%Most of the continual learning approaches, especially the regularization approaches, require a large number of examples to achieve high performance on each new task and %approximate the importance of each parameter. When there are only a few examples for training, they can't achieve high performance and have deviation on the importance of %each parameter which cause they also can't retain the old knowledge.

These related works presented solutions to the continual learning problem, whose setting is quite different from that of the
few-shot learning
% \Red{few-shot learning}
problem. Hence, none of them can be directly applied to
few-shot learning
% \Red{few-shot learning}
tasks.



==> Continual Few-Shot Learning_Arxiv/4-Methodology.tex <==
%=========================================================
\section{Problem Statement}
\label{Sec:Problem}

In the regular machine learning setting for classification, we aim to train a model representing a function $F(\cdot)$
which maps the given samples $\bx$ to the output $y$. Usually we train the parameters $\btheta$ of the model
on $\bD_{train}$ and evaluate it on $\bD_{test}$. While in the few-shot learning setting, we are interested
in meta-sets $\mathscr{D}$ which contain multiple regular datasets, and each dataset $\bD \in \mathscr{D}$
is split into $\bD_{train}$ and $\bD_{test}$ as those in regular machine learning.

% \Red{Since the proposed CML is based on MAML}~\cite{Finn2017} 
% \Red{which follows the meta-learning framework to deal with the few-shot learning, we would like to formulate the continual few-shot learning in the meta-learning framework similarly.}
% \Blue{CML, following meta-learning framework, focuses on continual few-shot learning tasks,}

% \Red{In the meta-learning framework for the few-shot learning problem}, 
In the few-shot learning problem,
%
we have meta-sets $\mathscr{D}_{meta-train}$ and $\mathscr{D}_{meta-test}$ used during
\emph{meta-training} and \emph{meta-testing} phases respectively~\cite{Ravi2017}.
%
It is important that the class labels in $\mathscr{D}_{meta-train}$ are not overlapping
with those of $\mathscr{D}_{meta-test}$.
%
% We consider $N$-way, $K$-shot tasks. 
%
Considering $N$-way, $K$-shot classification, for each task $\mathcal{T}_{i}$ with dataset $\bD \in \mathscr{D}$,  
% In each $\bD \in \mathscr{D}$,
$\bD_{train}$ contains $K$ samples
for each of $N$ classes, and $\bD_{test}$ contains samples for evaluation.
%
During the meta-training phase, we aim to train a meta-learner on $\mathscr{D}_{meta-train}$, 
which takes $\bD$ as input and then
produces a learner (with parameters $\btheta$) to maximize its classification accuracy
on the corresponding $\bD_{test}$. 
%
% \Red{Note that \sout{the} $\bD_{test}$ is also used to optimize the meta-learner.}
In contrast to regular machine learning, $\bD_{test}$ is used in the optimization.
We evaluate the performance of meta-learner on $\mathscr{D}_{meta-test}$ during the meta-testing phase.

In the continual learning setting, different tasks arrive in a sequence $[\mathcal{T}_1 \dots \mathcal{T}_n]$.
%
%and each task has class labels that are not overlapping with those of other tasks.
%
The most challenging part is that when training a new task $\mathcal{T}_j$, only $\bD_{train}$ of $\mathcal{T}_j$
is accessible, while $\bD_{train}$ of any previous task $\mathcal{T}_i$ $(i < j)$ is unavailable.
%not available.

Here, we study a new continual few-shot learning problem,
%. In this problem, 
%
where we have the meta-sets
consisting of $\mathscr{D}_{meta-train}$ and $\mathscr{D}_{meta-test}$,
% \Blue{performing N-way, K-shot learning on task set $\mathcal{T}$}, 
which are the same as those of the few-shot learning problem.
%\sout{just as those in} the few-shot learning setting.  
%
% We also have the same meta-training phase.
Similarly, the learning can be divided into the meta-training and meta-testing;
%
however, during the meta-testing, 
instead of arriving in a batch like the few-shot learning, tasks arrive sequentially.
%tasks arrive sequentially
% one by one in a sequence
%\Red{like the continual learning} rather than batchfully
%in a batch 
%\Red{like the few-shot learning}.
Moreover, in contrast to the continual learning,
each new task $\mathcal{T}_i$ only has a few samples (e.g., 5) in $\bD_{train}$ for each class.
%
Besides, we have prior knowledge (i.e., $\mathscr{D}_{meta-train}$), which can contribute to the meta-testing.
% to the learning of sequentially arrived tasks.
%
%there is a meta-set $\mathscr{D}_{meta-train}$ which can be regarded as prior knowledge to help .
%
We believe that this problem setting is more realistic and can better represent the process
of continuously learning new concepts of a human.  The main challenge is to ensure that the learner can quickly, effectively and continuously learn new concepts without forgetting what it has already learned.
%
% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.33]{CML_overview.png}
% \caption{Overview of Continual Meta-Learner(CML)}
% \label{Fig:CML}
% \end{figure}

%---------------------------------------------------------

%=============================================================================
\section{Continual Meta-Learner (CML)}
\label{Sec:Method}
%==============================================================================
%In this section, we firstly give an overview of CML and then
%describe the algorithm for training CML in details.
%The major notations are summarized in Table~\ref{Tab:Notations}.

%==============================================================================
\subsection{Overview}
%==============================================================================
% \sout{As illustrated in Figure~\ref{Fig:CML},}
%
% During the meta-testing phase, tasks arrive \Blue{in a sequence}.
% % one by one in a sequence.
% Each time when a new task $\mathcal{T}_i$ arrives,
% % For each task $\mathcal{T}_i$ \Red{consisting of \sout{a} $\bD_{train}$ and \sout{a} $\bD_{test}$}, 
% %
% CML uses images from $\bD_{train}$ to quickly learn to handle the new task,
% %
% and then takes images from $\bD_{test}$ as input and outputs the corresponding class labels.
%
As illustrated in Figure~\ref{Fig:CML}, during the meta-testing phase, tasks arrive one by one in a sequence.
Every time when a new task $\mathcal{T}_i$ arrives, CML uses images from $\bD_{train}$ to quickly learn to handle the new task
and then takes images from $\bD_{test}$ as input and outputs the corresponding class labels.
CML consists of the following core components:

1) Teacher Network $F_{\btheta_t}(\cdot)$: It takes an image $\bx$ as input and extracts its features to form a feature map $\bM_t$ with a dimension $z$.
% which are then pushed to the Classifier $P(\cdot)$ and the Discriminator $D_{\btheta_d}(\cdot)$.

2) Student Network $G_{\btheta_s}(\cdot)$: 
%
As the core part of CML, it takes $\bD_{train}$ as input
%all training images 
and generates an \emph{all-class} matrix $\bV$.
Each row of $\bV$ corresponds to a class vector $\bV^l$ with dimension $z$,
% a dimension of $z$, 
which can be considered as 
% a representation of images of the $l^{th}$ class.
a representation of $l^{th}$ class.

3) Classifier $P(\cdot)$: It takes the image feature map $\bM_t$ and the all-class matrix $\bV$ as input and predicts the class of image.
% which class \Blue{the} image belongs to.
%
% In addition, it is responsible for storing $\bV$ during the meta-testing phase.

% 4) Discriminator $D_{\btheta_d}(\cdot)$: It tries to distinguish between 
% the image feature map $\bM_t$
% %the feature map of an image 
% (belonging to class $l$) and the corresponding class vector $\bV^l$. 
% %
% Note that it is only used during the meta-training phase to guide the Student Network for better class vectors.
%
4) Class Storage Module (CSM): It stores $\bV$ of all previous tasks in a pair form of label and class vector $\langle y^l, \bV^l\rangle$, which are used to overcome catastrophic forgetting.

% \sout{As illustrated in Figure~\ref{Fig:CML},}
In addition, we introduce a Discriminator $D_{\btheta_d}(\cdot)$: 
It tries to distinguish between the image feature map $\bM_t$ (belonging to class $l$) 
and the corresponding class vector $\bV^l$ during the meta-training phase. 
It is trained with the Student Network in an adversarial manner and can guide the Student Network for better class vectors. 

When a new task $\mathcal{T}_i$ arrives during the meta-testing phase,
CML takes $\bD_{train}$ as input, and performs \textit{fast-learning}
%, which will be discussed \Blue{later in detail}.
%
% \sout{During fast-learning, we train the student network by minimizing \sout{both} the loss $\ell_{s,p}$ on the classifier and the loss $\ell_{s,d}$ on the discriminator.}
%
% After fast-learning, the student network 
to generate the all-class matrix $\bV$ 
% for current task $\mathcal{T}_i$ 
and 
% the classifier 
stores $\bV$ in Class Storage.
% in a pair form of label and class vector $\langle y^l, \bV^l\rangle$.
When evaluating with $\bD_{test}$, the Teacher Network generates the feature map $\bM_t$ for each input image $\bx$,
and passes $\bM_t$ to the Classifier
%.
% \sout{and the corresponding all-class matrix $\bV$ is retrieved from the memory.}
%
% Then the classifier is used 
to predict the class of image
% for the input image $\bx$ 
by calculating the similarity between 
% its feature map 
$\bM_t$ and
each class vector $\bV^{l}$ in $\bV$ learned from the fast-learning.
% \Red{stored in itself}.
%
The design of CML leads to the following desirable properties:

1) \textit{Learning quickly and effectively from a few samples}: CML learns a good initialization of the Student Network
after the meta-training phase such that it can adapt to any new task with only a few samples. Moreover,
the Student Network and the Discriminator are trained in an adversarial manner such that the generated class vectors
are close to the best ones, which is the key to accurate classification.

2) \textit{Overcoming catastrophic forgetting}: Even though the new tasks come in a continual manner, CML learns to handle each new task independently with the same good initialization (i.e., $\btheta$),
% from the same good initialization, 
which would not reduce the performance of the former tasks or interfere with the learning for new tasks.
% for the future tasks.} 
To conquer the catastrophic forgetting, CML stores the all-class matrix $\bV$ in the Class Storage Module (CSM), which can be retrieved when needed, i.e., will not be forgotten.
Moreover, it only needs a small memory footprint.
% \sout{CML conquers catastrophic forgetting in a rather direct way by storing the all-class matrix $\bV$ in the memory} 


3) \textit{Model-agnostic}: As MAML, CML can be applied to any model that can be trained by gradient descent.

%=====================================================================================================================

\begin{algorithm}[t]
\caption{Meta-training Algorithm for CML}
\label{Alg:CML}

{\bf Require:} The pre-trained Teacher Network $F_{\btheta_t}(\cdot)$ \\
{\bf Require:} Task distribution $p(\mathcal{T})$ \\
{\bf Require:} $\alpha_s/\alpha_d, \beta_s/\beta_d$: the step sizes for fast-learning and meta-update respectively
\begin{algorithmic}[1]
\STATE Randomly initialize $\bm\btheta_s, \bm\btheta_d$;
\WHILE{not done}
\STATE Sample a batch of tasks $\mathcal{T}_i \sim p(\mathcal{T})$;

\FORALL{$\mathcal{T}_i$}
%\STATE Sample $N \times K$ training examples $\bD_{train} = \{(\bx_1, y_1), \dots, (\bx_k, y_k)\}$ from $\mathcal{T}_i$
\STATE Obtain $\bD_{train}$ from $\mathcal{T}_i$;
\STATE all-class matrix $\bV_i \gets G_{\btheta_s}(\bx)$ where $\bx \in \bD_{train};$
%\STATE $\bV \gets G_{\btheta_s}(\bx | \bx \in \bD_{train})$;
\STATE $\mathcal{L}_{train}^s (\btheta_s) \gets \frac{1}{|\bD_{train}|} \sum\limits_{(\bx, y) \in \bD_{train}} \ell_{s}(\btheta_s; \bx, y, \bV_i)$;
\STATE $\btheta_{i,s}^{'} \gets \btheta_s - \alpha_s \nabla_{\btheta_s} \mathcal{L}_{train}^s(\btheta_s)$;
%\STATE $\bV^{'} \gets G_{\btheta_{i,s}^{'}}(\bx | \bx \in \bD_{train})$;
\STATE $\mathcal{L}_{train}^d(\btheta_d) \gets \frac{1}{|\bD_{train}|} \sum\limits_{\bx \in \bD_{train}} \ell_d(\btheta_d;\bx)$;
\STATE $\btheta_{i,d}^{'} \gets \btheta_d - \alpha_d \nabla_{\btheta_d} \mathcal{L}_{train}^d (\btheta_d)$;

\STATE all-class matrix $\bV_{i}^{'} \gets G_{\btheta_{i,s}^{'}}(\bx)$ where $\bx \in \bD_{train};$
% \STATE Obtain $\bD_{test}$ from $\mathcal{T}_i$;
% \Red{\STATE $\mathcal{L}_{test}^s(\btheta_{i,s}^{'}) \gets \frac{1}{|\bD_{test}|} \sum\limits_{(\bx, y) \sim \bD_{test}} (\ell_{s, p}(\btheta'_{i,s}; \bx, y) + \ell_{s,d}(\btheta'_{i,s};\bx))$ ;}

% \Red{\STATE $\mathcal{L}_{test}^s(\btheta_{i,s}^{'}) \gets \frac{1}{|\bD_{test}|} \sum\limits_{(\bx, y) \sim \bD_{test}} \ell_{s, p}(\btheta'_{i,s}; \bx, y) + \frac{1}{N}
% \sum\limits_{l=1}^N \ell_{s,d}(\btheta_s;l)$ ;}
\ENDFOR

\FORALL{$\mathcal{T}_i$}
% \STATE Obtain $\bD_{train}$ from $\mathcal{T}_i$;
% \STATE $\mathcal{L}_{train}^d(\btheta_d) \gets \frac{1}{|\bD_{train}|} \sum\limits_{\bx \sim \bD_{train}} \ell_d(\btheta_d;\bx)$;
% \STATE $\btheta_{i,d}^{'} \gets \btheta_d - \alpha_d \nabla_{\btheta_d} \mathcal{L}_{train}^d (\btheta_d)$;
%\STATE Sample test examples $\bD_{test} = \{(\bx_1, y_1), \dots, (\bx_k, y_k)\}$ from $\mathcal{T}_i$
\STATE Obtain $\bD_{test}$ from $\mathcal{T}_i$;
\STATE{$\mathcal{L}_{test}^s(\btheta_{i,s}^{'}) \gets \frac{1}{|\bD_{test}|} \sum\limits_{(\bx, y) \in \bD_{test}} (\ell_{s}(\btheta'_{i,s}; \bx, y, \bV_{i}^{'}) + \ell_{d}^-(\btheta'_{i,s};\bx));$}

\STATE $\mathcal{L}_{test}^d(\btheta_{i,d}^{'}) \gets \frac{1}{|\bD_{test}|} \sum\limits_{\bx \in \bD_{test}} \ell_d(\btheta_{i,d}^{'};\bx)$;

\ENDFOR
\STATE $\btheta_s \gets \btheta_s - \beta_s \nabla_{\btheta_s} \sum_{\mathcal{T}_i} \mathcal{L}_{test}^s(\btheta_{i,s}^{'})$;

\STATE $\btheta_d \gets \btheta_d - \beta_d \nabla_{\btheta_d} \sum_{\mathcal{T}_i} \mathcal{L}_{test}^d(\btheta_{i,d}^{'})$;

\ENDWHILE

\end{algorithmic}
\end{algorithm}

\subsection{Meta-training}
%====================================================================================================================
% We formally present the algorithm for training CML during \textit{meta-training} as Algorithm \ref{Alg:CML}.
We formally present the proposed CML as Algorithm \ref{Alg:CML} for \textit{meta-training}.
%
% Before meta-training,
In the beginning, we pre-train a teacher network
% Teacher Network $F_{\btheta_t}(\cdot)$ 
on the meta-set $\mathscr{D}_{meta-train}$ such that it gains enough knowledge to serve
as a ``teacher".
%
%
% After we pre-train this network, 
After pre-training, we discard the last fully-connected layer and
keep the the remaining network
as the Teacher Network, whose parameters $\btheta_t$ will be fixed during the meta-training and the meta-testing phases. 

During the meta-training phase, CML takes a batch of tasks $\{\mathcal{T}_1, \cdots, \mathcal{T}_n\}$ 
($n=4$ in our implementation) as input
and learns a good initialization of the Student Network and the Discriminator.
%
The entire meta-training consists of two phases: \textit{fast-learning} and \textit{meta-update}. \\
% \sout{During the fast-learning (lines 4-10), CML learns from $\bD_{train}$ of each individual task of the batch;
% while during the meta-update (lines 11-17), it learns from $\bD_{test}$ across all tasks of the batch.}
%
%

\noindent \textbf{Fast-learning} \qquad
% \Blue{is performed by CML for $\bD_{train}$ of each task in the batch (Line 4-12).}
CML learns from $\bD_{train}$ of each
individual task in the batch (Line 4-12).
%
Given an input image $\bx$ ($84 \times 84$ in our implementation),
the Teacher Network
% teacher network 
yields a feature map $\bM_t$ with a dimension $z$, and the Student Network yields a feature map $\bM_s$ with the same dimension.
% \sout{Given all input images $\bx$ of class $l$,
% the Student Network yields a class vector $\bV^l$ with the same dimension $z$.}
%
% In the 1-shot setting,
For the 1-shot setting, we directly obtain the class vector $\bV^l$ for the input image belongs to the $l^{th}$ class, i.e., $\bV^l=\bM_s$.
% if the input image belongs to the $l^{th}$ class, we then directly obtain class vector $\bV^l$.
%
% In the K-shot setting,
For the K-shot setting,
we obtain the class vector $\bV^l$ by taking the mean values.
%
% By doing so, we ensure that the feature map $\bM$ and each class vector $\bV^l$ have the same dimension.
% \Blue{By doing so, we ensure the same dimension of the feature map $\bM$ and each class vector $\bV^l$}.
%
The all-class matrix $\bV$ is then constructed by stacking the class vectors all together.
%
$\bV$ has a dimension of $N \times z$, where $N$ is the number of classes ($N=5$ in our implementation) and $z$ is the dimension of each class vector $\bV^l$ ($z=512$ in our implementation).
%
% \Red{Note that the subscript $i$ of $\bV$ in Algorithm~\ref{Alg:CML} is the task index rather than the class label $l$.}
%
%
% \sout{After fast-training for each new task, CML stores the corresponding all-class matrix $\bV$ in the memory.
% Note that each class vector only needs a very small space of 4KB because they are
% 512 64-bits numbers.
% Hence CML has a low memory footprint.}
%
%And we can continue to reduce memory consumption by reducing the dimension $z$ of each class vector $\bV^l$.}

Then Classifier calculates the cosine similarity between 
% $\bM$ of image $\bx$ 
the feature map $\bM_t$
and each class vector $\bV^l$ 
% as the prediction score for each class:
for the prediction score of each class:
%{like~\cite{Gidaris2018,Qi2018}}
%
\begin{align}
\label{Equatio: classifier}
    P(\bM_t, \bV) = \text{softmax}(Cos(\bM_t, \bV^{\top})),
\end{align}
where $Cos(\cdot)$ calculates the cosine similarity.
%
We choose the cosine similarity because it eliminates the interference
resulting from different orders of magnitude corresponding to different classes.
%
%If we use the dot-product of $\bM$ and $\bV^l$ directly, the score may be high
%\Red{even if they are in different directions because of the huge magnitudes of them.}
%
After that, we use a softmax function to normalize prediction scores.

To train the Student Network during the fast-learning, we use the cross-entropy loss $\ell_{s}$ on the Classifier:
%
% \begin{align}
% \label{Equation: ell_sp}
%     \begin{split}
%     \ell_{s,p}(\btheta_s; \bx, y) = - [y \log P(F_{\btheta_t}(\bx), G_{\btheta_s}(\bX)) \\
%     + (1-y) \log (1-P(F_{\btheta_t}(\bx), G_{\btheta_s}(\bX)))],
%     \end{split}
% \end{align}
\begin{align}
\label{Equation: ell_sp}
    \begin{split}
    \ell_{s}(\btheta_s; \bx, y, \bV) = - [y \log P(F_{\btheta_t}(\bx), \bV) \\ 
    + (1-y) \log (1-P(F_{\btheta_t}(\bx), \bV))],
    \end{split}
\end{align}
%
where $(\bx, y)$ is an image/label pair from $\bD_{train}$ 
% \sout{and $\bX$ is the corresponding set of images}
% \sout{$G_{\btheta_s}(\bX)$ actually gives the all-class matrix $\bV$.}
and $\bV$ is the all-class matrix.

%--------


%
%
%This is why we integrates the Adversarial Learning into our model.
%

% We train the student network
The Student Network is trained by minimizing the loss $\ell_{s}$ through gradient descent (Line 6-8).
%for several steps (5 steps in our experiments).
%
Note that it is trained for each task $\mathcal{T}_i$ independently but
% starts from the same parameters $\btheta_s$.
with the same parameters $\btheta_s$.
%
% After fast-learning, the parameters $\btheta_s$ are updated to $\btheta_{i,s}^{'}$ for each task $\mathcal{T}_i$.
Through fast-learning, $\btheta_{i,s}^{'}$ is calculated for each task $\mathcal{T}_i$ based on $\btheta_s$.
%
%and the student network generates the corresponding all-class matrix $\bV^{'}$ (line 9).
%
%
% Note that the $i$ here doesn't refer to the $i^{th}$ class, but the task $\mathcal{T}_i$.

%For the training of Discriminator $D_{\btheta_d}(\cdot)$ in \textit{fast-learning}.
The Discriminator takes the feature map $\bM_t=F_{\btheta_t}(\bx)$ from the Teacher Network
as the real (i.e., true) input and the feature map $\bM_s=G_{\btheta_s}(\bx)$ from the Student Network as the fake (i.e., false) input. Its loss $\ell_d$ is:
% \begin{align}
% \label{Equation: ell_d}
%     \begin{split}
%     \ell_d(\bx) = - & \sum_{\bx \sim \bD_{train}} [ \log D_{\btheta_d}(F_{\btheta_t}(\bx)) \\
%     & + \log (1-D_{\btheta_d}(G_{\btheta_s}(\bx)))];
%     \end{split}
% \end{align}
\begin{align}
\label{Equation: ell_d}
    % \begin{split}
    % \ell_d(\btheta_d;\bx) = - [ \log D_{\btheta_d}(F_{\btheta_t}(\bx)) \\
    % + \log (1-D_{\btheta_d}(G_{\btheta_s}(\bx)))],
    % \end{split}
    \ell_d(\btheta_d;\bx) = - (\ell_d^+(\btheta_d;\bx) + \ell_d^-(\btheta_d;\bx))
\end{align}
where 
\begin{align}
    \label{Equation: ell_d_pos}
    \ell_d^+(\btheta_d;\bx) &= \log D_{\btheta_d}(F_{\btheta_t}(\bx)),  \\
    \label{Equation: ell_d_neg}
    \ell_d^-(\btheta_d;\bx) &= \log (1-D_{\btheta_d}(G_{\btheta_s}(\bx))),
\end{align}
and $\bx$ is an image from $\bD_{train}$. 
% \sout{and the image vector $G_{\btheta_s}(\bx)$ is the output of the Student Network with input $\bx$}
% before taking the mean if $K > 1$}.
%
% \sout{Similar to the student network, the discriminator is also trained in an adversarial manner.}
Similar to the Student Network,
% its parameters $\btheta_d$ are updated to $\btheta_{i,d}^{'}$ after the fast-learning phase (line 9-10).
$\btheta_{i,d}^{'}$ is calculated based on $\btheta_d$ through fast-learning (Line 9-10).

% \Red{Since the overall learning ability in fast-learning is limited, e.g., 1 sample for each of 5 steps, }
% 
The small amount of training data and gradient descent steps (e.g., 1 sample and 5 steps) lead to a limited learning ability of fast-learning.
%
In such kind of condition, during the fast-learning phase, the Student Network should devote into the classification task (i.e., $\ell_{s}$), rather than interfered by the adversarial training. 
%
As discussed above, the adversarial loss (i.e, $\ell_d$) is only used to train the Discriminator in fast-learning.
% we believe that the Student network should devote into the classification task, an adversarial loss should not be involved during the fast-learning of the Student network.

% \Red{After fast-training for each new task, CML stores the corresponding all-class matrix $\bV$ in the Classifier in a pair form of label and class vector $\langle y^l, \bV^l\rangle$.
% Note that each class vector only needs a very small space of 4KB because they are 512 64-bits numbers. Hence CML has a low memory footprint.} 
Through fast-learning phase, for each task, CML stores its all-class matrix $\bV$ in a pair form of label and class vector $\langle y^l, \bV^l\rangle$, which only consumes a very small space of 12KB. Hence CML has a low memory footprint.\\


%-----------------------------------------------------------------
\begin{table*}[htbp]\scriptsize
\centering
\caption{Classification accuracies for 4 tasks at the end of the sequence on MiniImageNet (5-way, 1-shot)}
% \normalsize
\renewcommand\arraystretch{1.3}
\begin{tabular}{l|cccc|c}
\toprule
Method & $\mathcal{T}_1$ & $\mathcal{T}_2$ & $\mathcal{T}_3$ & $\mathcal{T}_4$ & Average \\ \midrule
MAML~\cite{Finn2017}+FT & $26.85\pm1.62\%$ & $27.84\pm1.60\%$ & $30.61\pm1.63\%$ & $34.42\pm1.50\%$ & $29.93\%$\\ 
MAML~\cite{Finn2017}+MAS~\cite{Aljundi2018} & $27.20\pm1.52\%$ & $27.99\pm1.61\%$ & $31.60\pm1.62\%$ & $34.45\pm1.60\%$ & $30.31\%$ \\ 
MN~\cite{Vinyals2016}+CSM & $43.01\pm1.14\%$ & $43.54\pm1.17\%$ & $43.18\pm1.18\%$ & $43.31\pm1.21\%$ & $43.26\%$ \\ 
PN~\cite{Snell2017}+CSM & $48.19\pm0.87\%$ & $48.63\pm0.91\%$ & $48.39\pm0.83\%$ & $48.57\pm0.88\%$ & $48.44\%$ \\ \cmidrule(lr){1-6}
% CML(Ours) / D & $56.40\pm1.56\%$ & $57.01\pm1.54\%$ & $56.89\pm1.53\%$ & $57.33\pm1.55\%$ & $56.91\%$ \\ \hline
CML(Ours) & \bm{$57.86\pm1.47\%$} & \bm{$60.70\pm1.42\%$} & \bm{$57.85\pm1.49\%$} & \bm{$58.23\pm1.38\%$} & \bm{$58.66\%$} \\ \bottomrule

\end{tabular}
\label{mini-1shot}
\end{table*}

%-----------------------------------------------------------------
\begin{table*}[htbp]\scriptsize
\centering
\caption{Classification accuracies for 4 tasks at the end of the sequence on MiniImageNet (5-way, 5-shot)}
\renewcommand\arraystretch{1.3}
\begin{tabular}{l|cccc|c}
\toprule
Method & $\mathcal{T}_1$ & $\mathcal{T}_2$ & $\mathcal{T}_3$ & $\mathcal{T}_4$ & Average \\ \midrule
MAML~\cite{Finn2017}+FT & $29.74\pm1.91\%$ & $29.02\pm1.76\%$ & $34.04\pm1.80\%$ & $49.34\pm1.60\%$ & $35.53\%$ \\
MAML~\cite{Finn2017}+MAS~\cite{Aljundi2018} & $28.97\pm1.71\%$ & $26.92\pm2.00\%$ & $35.09\pm1.90\%$ & $50.52\pm1.61\%$ & $35.37\%$ \\
MN~\cite{Vinyals2016}+CSM & $53.68\pm1.02\%$ & $54.11\pm0.98\%$ & $54.13\pm1.03\%$ & $53.77\pm1.02\%$ & $53.92\%$ \\
PN~\cite{Snell2017}+CSM & $66.08\pm0.72\%$ & $66.80\pm0.73\%$ & $66.16\pm0.71\%$ & $66.78\pm0.72\%$ & $66.45\%$ \\ \cmidrule(lr){1-6}
% CML(Ours) / D & $69.30\pm1.38\%$ & $69.95\pm1.25\%$ & $69.17\pm1.28\%$ & $69.96\pm1.33\%$ & $69.60\%$ \\ \hline
CML(Ours) & \bm{$70.86\pm1.68\%$} & \bm{$70.85\pm1.55\%$} & \bm{$71.09\pm1.65\%$} & \bm{$69.11\pm1.81\%$} & \bm{$70.48\%$} \\ \bottomrule

\end{tabular}
\label{mini-5shot}
\end{table*}


\noindent \textbf{Meta-update} \qquad
% We train both the Student network and the Discriminator (lines 13-19) on $\bD_{test}$ (rather than $\bD_{train}$).
Both of the Student Network and the Discriminator are trained on $\bD_{test}$ across all tasks during meta-update (Line 18-19) to arrive a good initialization from where a new task can be handled with a few samples (e.g., 1 or 5).
%
% For the meta-update of the Student network (line 18), we use the same cross-entropy loss $\ell_{s,p}$ (Equation~\ref{Equation: ell_sp})
% as that during fast-learning.

For the Student Network, during meta-update, the cross-entropy loss $\ell_{s}$ (Equation~\ref{Equation: ell_sp}, Line 15) for classification is computed based on images $\bx$ from $\bD_{test}$ and the updated all-class matrix $\bV^{'}$ through the fast-learning.
% In addition, an adversarial loss $\ell_{s,d}$ is added (Line 15),
In addition, the same adversarial loss $\ell_d(\btheta_d;\bx)^-$ as Equation~\ref{Equation: ell_d_neg} is added (Line 15).
%
% \Red{
% Besides the loss $\ell_{s,p}$ corresponding to the Classifier, we add another loss $\ell_{s,d}$ corresponding to the Discriminator (line 15).
%
% \Blue{For the Discriminator, the binary-entropy loss $\ell_{s,d}$ is used (Line 16),
% 
% with $\bM_s=G_{\btheta_s}(\bx)$ as input, 
%
% to calculate the probability of being a true sample.
% The Discriminator takes each image vector $G_{\btheta_s}(\bx)$ as input, calculates the probability of the input being a true sample.
% We use the binary-entropy loss $\ell_{s,d}$:
%
% The binary-entropy loss $\ell_{s,d}$ is defined as:
% \begin{align}
% \label{Equation: ell_sd}
%     \begin{split}
%     \ell_{s,d}(\btheta_s;\bx) = - \log D_{\btheta_d}(G_{\btheta_s}(\bx)),
%     \end{split}
% \end{align}
% where $\bx$ is an image from $\bD_{test}$.
% and the feature map $\bM_s$ is same as that in the fast learning.
%}
% \sout{where $G_{\btheta_s}(\bX)$ actually gives the all-class matrix $\bV$ of $\bD_{test}$ and $R(\bV,l)$ returns the $l^{th}$ row of $\bV$, i.e., $\bV^l$.}
%
Similar to the Generative Adversarial Networks (GANs)~\cite{Goodfellow2014}, 
the Student Network can
% be considered as
be considered a generator to generate the feature maps $\bM_s$.
Meanwhile, the Discriminator is used to distinguish between $\bM_s$ and $\bM_t$, which is generated by the Teacher Network.
% distinguish each feature map $\bM_s$ generated by the Student Network from true samples generated by the Teacher Network, when training the Student Network.}
%

For the meta-update of the Discriminator, we use the same binary-entropy loss $\ell_d$ (Equation~\ref{Equation: ell_d}, Line 16) given the images $\bx$ in $\bD_{test}$.

The meta-update of the proposed meta-training algorithm can %guide the Student Network to achieve a better initialization, from which, 
% through fast-learning, a more representative and discriminative all-class matrix $\bV$ can be obtained. 
lead to a more representative and discriminative all-class matrix $\bV$ during meta-testing,
%through fast-learning,
%
which is contributed by two factors:
%
1) The Teacher Network, through pre-training on the meta-set $\mathscr{D}_{meta-train}$, can generate a good feature map $\bM_t$ for each image $\bx$, which serves as a learning template for the Student Network.
%
2) In contrast to $\bD_{train}$, the $\bD_{test}$ used in the meta-update consists of more samples for each class (e.g., 15), 
% 
which does not have the limitation of few-shot setting in the fast-learning phase.
Thus the adversarial training, by adding the adversarial loss (i.e., $\ell_{d}^-$) during the meta-update, 
% instead of interfering with the fast-learning phase due to the limitation of few-shot setting, 
can guide the Student Network to achieve a better initialization from where a more discriminative matrix can be obtained.
% \Red{Since there are more samples in $\bD_{test}$ than $\bD_{train}$, e.g., 15 samples per class, adversarial learning in meta-update can subtly avoid the limitation of few-shot setting in $\bD_{train}$.
%
% Thus, with more samples, the Discriminator can guide the Student Network to arrive at a better initialization from where a more representative and discriminative all-class matrix $\bV$ can be obtained through the fast-learning.
%
As a matter of course, a better all-class matrix $\bV$ stands for higher classification accuracy for each new task during the meta-testing.
%
%  from which each new task could be easily and quickly solved.}
% \sout{The Student Network can be considered as a generator used to generate the all-class matrix $\bV$.}
%
% \sout{Similar to the GAN~\cite{Goodfellow2014}, the Discriminator here
% helps the Student Network generate a more representative all-class matrix via adversarial learning.}
%
On the other hand, the cross-entropy loss $\ell_{s}$ for classification can stabilize the adversarial training of the Student Network and the Discriminator. 
% 
% In addition, it can alleviate mode collapse, which is common problem in GANs training.}
% Furthermore, the cross-entropy loss $\ell_{s,p}$ for classification can make training the Student Network and the Discriminator more stable, and prevent model collapses.
% %
% This is because the loss $\ell_{s,p}$ can still improve the Student Network even when the Discriminator makes a mistake;
% and then the improvement on the Student Network can help train the Discriminator.
% %
% Hence, the losses $\ell_{s,p}$ and $\ell_{s,d}$ benefit from each other.
Hence, in the meta-update, $\ell_{s}$ and $\ell_{d}^-$ can benefit from each other.


%
%\Red{While $\bV$ is $\bV^{'}$ which is generated by the updated model $G_{\btheta_{i,s}^{'}}(\cdot)$.}
%
%$(x,y)$ are an image-label pair from $\bD_{test}$ for each task $\mathcal{T}_i$.
%
% We optimize the Student Network parameters $\btheta_s$ using gradient descent for just one step (line 18).
%
%
% We then use gradient descent to optimize its parameters $\btheta_d$ (line 19).
%
One-step gradient descent is performed on $\btheta_s$ and $\btheta_d$ to update the Student Network and the Discriminator respectively (Line 18-19).
%
Similar to the MAML~\cite{Finn2017}, 
% we perform the meta-update 
meta-update is performed
on the parameters $\btheta_s$ and $\btheta_d$ rather than $\btheta_{i,s}^{'}$ and $\btheta_{i,d}^{'}$,
%
while the losses $\ell_{s}$, $\ell_{d}^-$ and $\ell_d$ are computed based on the calculated
% by the updated 
parameters $\btheta_{i,s}^{'}$ and $\btheta_{i,d}^{'}$ 
%after 
through
fast-learning.
%
Note that the losses for meta-update are computed across all the tasks $\{\mathcal{T}_1, \cdots, \mathcal{T}_n\}$ in the batch rather than a single task.
In this way, CML can learn a good initialization of both the Student Network and the Discriminator such that
it can quickly learn to deal with a new task during the meta-testing phase.
%The student network and the discriminator are trained alternately in Algorithm~\ref{Alg:CML}.

%======================================================================================================================


%======================================================================================================================

\subsection{Meta-testing}
%====================================================================================================================
During the meta-testing phase,
%
we have $\btheta_{s}$ of the Student Network 
%and $\btheta_{d}$ of the Discriminator 
as a good initialization to handle the new tasks.
% we obtain $\btheta_{s}$ for the Student Network and $\btheta_{d}$ for the Discriminator trained from the meta-training phase as good initializations for handling a new arriving task. 
%
Note that the Discriminator is discarded, 
% since, during the meta-training phase, 
since it is only used to assist the training of the Student Network in the meta-update, rather than the fast learning, during the meta-training phase.
% And we discard the Discriminator since it is only used to guide the all-class matrix $\bV$ generation during the meta-training phase.}

As mentioned in Section 3, for continual few-shot learning, tasks arrive sequentially during the meta-testing phase.
For the new task in sequence,
%
similar to the meta-training phase,
the Student Network has the same fast-learning process 
% during the meta-training 
for quickly learning from the initialization $\btheta_{s}$ with a few samples. 
%
Through the fast-learning on $\bD_{train}$, the Student Network with the calculated parameters $\btheta_{s}^{'}$ generates an all-class matrix $\bV$ for the current task
%
and falls back to the initialization $\btheta_{s}$ for the next task. 
%
Then, for an image from $\bD_{test}$, with the feature map $\bM_t$ generated from the fixed Teacher Network,
the Classifier predicts which class the image belongs to, and stores the all-class matrix $\bV$ in a pair form of label and class vector $\langle y^l, \bV^l\rangle$ into the Class Storage Module (CSM).
%
% When inferring on an old tasks, 
When performing inference on a former task without accessible $\bD_{train}$ for the continual few-shot learning,
the Classifier retrieves the pairs $\langle y^l, \bV^l\rangle$ from the CSM according to the class labels of the former task and forms an all-class matrix $\bV$ for the task, which is used to predict the class of the images from $\bD_{test}$.
% There are three advantages \Blue{of} this memory-based mechanism:}

In this way, for each new task, the Student Network of CML always learns from the same initialization $\btheta_{s}$ to generate the all-class matrix $\bV$, which is stored independently and can be retrieved accordingly. Hence, the inference on the new task does not affect that on the former task, and the catastrophic forgetting is conquered at the cost of a small memory footprint.
%
% \Red{1) Since the Student Network always learns from the same initialization $\btheta_{s}$, the fast-learning for the current task would not interfere with the all-class matrix $\bV$ of the old tasks and the fast-learning of the future tasks, i.e., the catastrophic forgetting is conquered at the cost of a small memory footprint.}


% \Red{2) The number of classes that the entire model can recognize is incremental if memory allows because we store class matrices for all tasks in the Classifier.}

% \Red{3) We don't need to store the updated Student Network after fast-learning for every coming task, and just save the initialization $\btheta_{s}$ of the Student Network and the pre-trained Teacher Network which can save a lot of memory.}


%======================================================================================================================

\subsection{Implementation Details}
%====================================================================================================================
For the Teacher Network, we use ResNet18 following~\cite{He2016}. 
Given an input image $\bx$ with a size of $84 \times 84$, the ResNet18 yields a feature map $\bM$ with a dimension of $z=512 \times 1 \times 1 = 512$.

The Student Network contains a Convolutional Neural Network (CNN) similar to that in~\cite{Finn2017},
which has 4 convolutional modules, each of which contains a $3 \times 3$ convolution layer followed by batch normalization~\cite{Ioffe2015}, a ReLU nonlinearity and $2 \times 2$ max pooling.
%
It has 64 filters in the first two convolutional layers and 128 filters in the last two convolutional layers.
Given an input image $\bx$ with a size of $84 \times 84$,
the Student Network yields a feature map $\bM$ with a dimension of $z=128 \times 2 \times 2 = 512$, which is same as ResNet18.

We use a multilayer perceptron (MLP)~\cite{Goodfellow2016} to implement the Discriminator, which contains two fully-connected layers.
The first fully-connected layer is followed by batch normalization and a ReLU nonlinearity; and the second fully-connected layer is followed by
the sigmoid function that normalizes output.

In addition, in our implementation, during fast-learning, we set the number of training steps to 5, and the learning rates $\alpha_s$
and $\alpha_d$ of both the Student Network and the Discriminator to 0.01.
%
During meta-update, the learning rates $\beta_s$ and $\beta_d$ of the Student Network and the Discriminator are set to 0.1 and 0.001 respectively,
which both decay rapidly with the epoch.

==> Continual Few-Shot Learning_Arxiv/5-Eval.tex <==
\section{Performance Evaluation}
\label{Sec:Eval}
%In this section, we first present the experimental settings and then the results and analysis.

%-----------------------------------------------------------------
\begin{table*}[t]\scriptsize
\centering
\caption{Classification accuracies for 4 tasks at the end of the sequence on CIFAR100 (5-way, 1-shot)}
\renewcommand\arraystretch{1.3}
\begin{tabular}{l|cccc|c}
\toprule
Method & $\mathcal{T}_1$ & $\mathcal{T}_2$ & $\mathcal{T}_3$ & $\mathcal{T}_4$ & Average \\ \midrule
MAML~\cite{Finn2017}+FT & $31.03\pm1.73\%$ & $33.25\pm2.12\%$ & $34.07\pm1.79\%$ & $40.31\pm1.84\%$ & $34.66\%$ \\ 
MAML~\cite{Finn2017}+MAS~\cite{Aljundi2018} & $31.47\pm1.90\%$ & $32.84\pm1.88\%$ & $34.45\pm1.72\%$ & $40.69\pm1.89\%$ & $34.86\%$ \\ 
MN~\cite{Vinyals2016}+CSM & $52.93\pm1.13\%$ & $51.66\pm1.38\%$ & $51.90\pm1.40\%$ & $51.74\pm1.34\%$ & $52.05\%$ \\ 
PN~\cite{Snell2017}+CSM & $49.38\pm0.87\%$ & $49.38\pm0.85\%$ & $48.38\pm0.85\%$ & $49.24\pm0.86\%$ & $49.09\%$ \\ \cmidrule(lr){1-6}
% CML(Ours) / D & $61.53\pm1.65\%$ & $60.15\pm1.50\%$ & $60.72\pm1.57\%$ & $61.42\pm1.64\%$ & $60.95\%$ \\ \hline
CML(Ours) & \bm{$61.57\pm1.58\%$} & \bm{$62.80\pm1.49\%$} & \bm{$61.06\pm1.63\%$} & \bm{$62.91\pm1.56\%$} & \bm{$62.08\%$} \\ \bottomrule
% CML(Ours) & \sout{\bm{$55.65\pm1.69\%$}} & \sout{\bm{$54.99\pm1.50\%$}} & \sout{\bm{$57.70\pm1.71\%$}} & \sout{\bm{$55.62\pm1.55\%$}} & \sout{\bm{$55.99\%$}} \\ \hline

\end{tabular}
\label{CIFAR-1shot}
\end{table*}

%-----------------------------------------------------------------
\begin{table*}[t]\scriptsize
\centering
\caption{Classification accuracies for 4 tasks at the end of the sequence on CIFAR100 (5-way, 5-shot)}
\renewcommand\arraystretch{1.3}
\begin{tabular}{l|cccc|c}
\toprule
Method & $\mathcal{T}_1$ & $\mathcal{T}_2$ & $\mathcal{T}_3$ & $\mathcal{T}_4$ & Average \\ \midrule
MAML~\cite{Finn2017}+FT & $29.24\pm2.01\%$ & $33.21\pm2.03\%$ & $40.34\pm1.76\%$ & $58.18\pm1.73\%$ & $40.24\%$ \\ 
MAML~\cite{Finn2017}+MAS~\cite{Aljundi2018} & $31.22\pm1.90\%$ & $33.48\pm1.95\%$ & $40.92\pm1.82\%$ & $57.42\pm1.68\%$ & $40.76\%$ \\ 
MN~\cite{Vinyals2016}+CSM & $66.27\pm1.13\%$ & $65.00\pm1.20\%$ & $65.69\pm1.06\%$ & $65.30\pm1.21\%$ & $65.56\%$ \\ 
PN~\cite{Snell2017}+CSM & $70.39\pm0.70\%$ & $70.03\pm0.70\%$ & $69.02\pm0.74\%$ & $69.64\pm0.68\%$ & $69.77\%$ \\ \cmidrule(lr){1-6}
% CML(Ours) / D & $71.94\pm1.21\%$ & $71.91\pm1.18\%$ & $72.20\pm1.29\%$ & $72.25\pm1.25\%$ & $72.08\%$ \\ \hline
CML(Ours) & \bm{$74.04\pm1.21\%$} & \bm{$74.91\pm1.17\%$} & \bm{$73.38\pm1.23\%$} & \bm{$73.79\pm1.33\%$} & \bm{$74.03\%$} \\ \bottomrule
% CML(Ours) & \sout{\bm{$71.57\pm1.59\%$}} & \sout{\bm{$70.10\pm1.68\%$}} & \sout{\bm{$70.86\pm1.64\%$}} & \sout{\bm{$71.08\pm1.65\%$}} & \sout{\bm{$70.09\%$}} \\ \hline

\end{tabular}
\label{CIFAR-5shot}
\end{table*}
%-----------------------------------------------------------------


%------------------------------------------------------------------------
\subsection{Experimental Setup}
\label{Sec:Setup}

In our experiments, we evaluated the proposed CML on two widely-used image datatsets, MiniImageNet~\cite{Vinyals2016} and CIFAR100~\cite{Krizhevsky2009}.
%
MiniImageNet includes 100 classes with 600 samples per class and each image has a spatial size of $84 \times 84$.
%
CIFAR100 is another image dataset, which also has 100 classes and each class contains 600 samples too.
%
Both datasets were divided into three disjoint meta-sets with 64, 16, and 20 classes for meta-training, meta-validation and meta-testing respectively.
%
%\Red{For MiniImageNet, we used the same split as~\cite{Gidaris2018} which sampled 300 extra images for validation and 300 extra images for testing in meta-set %$\mathscr{D}_{meta-train}$.
%For CIFAR100, since there are total 600 images for each class, we randomly sampled 400 images for trainging, 100 images for validatation and 100 images for testing.}
%
%We train CML following the settings given in~\cite{Finn2017}.
Following the settings used in~\cite{Finn2017}, each task was set to a $5$-way, $K$-shot ($K=1$ or $5$ in the experiments).
We firstly sampled $5$ classes from the meta-training dataset.
For each class, we sampled $K$ images for training and $15$ images for testing.
Then the training set $\bD_{train}$ includes $5K$ images and the testing set $\bD_{test}$ contains $15*5=75$ images.
%
%During the meta-training phase, we updated our model once for each batch of tasks from $\mathscr{D}_{meta-train}$.
%
During the meta-testing phase, tasks from the meta-testing set (with unseen classes) arrive one by one in a sequence.
%
%The settings during \emph{fast-learning} is as same as those in meta-training phase.
%
Whenever training for a new task $\mathcal{T}_j$ was completed, we also evaluated each method over
all the previous tasks $\{\mathcal{T}_i\} (\forall i<j)$ using their $\bD_{test}$.
%
% \Red{Here we used the metric \emph{Backward transfer} (BWT) following~\cite{Lopez2017}:
% \begin{align}
% \label{Equation: BWT}
%     \begin{split}
%     {\rm BWT} =  \frac{1}{T-1} \sum\limits_{i=1}^{T-1} R_{T,i}-R_{i,i},
%     \end{split}
% \end{align}
% where $T$ is the length of the task sequence, $R_{i,j}$ is the accuracu result on task $\mathcal{T}_j$ after trained on task $\mathcal{T}_i$. }

%
%without training their $\bD_{train}$ again.
%
%More specifically, we consider 5-way, 1-shot and 5-shot image classification tasks and the length of sequence of tasks in meta-test phases is 4.

We are the first to consider the continual few-shot learning problem, which cannot be solved directly by any existing few-shot learning or
continual learning method.
%
For the purpose of performance evaluation, we chose several recent and well-known meta-learners~\cite{Finn2017,Snell2017,Vinyals2016}
as the baselines and slightly modified them to handle the continual few-shot learning problem studied here.
%
%most of works which focus on continual learning or meta-learning can't be evaluated on Continual Meta-Learning problem directly. Thus we choose several related and %well-known methods~\cite{Finn2017, Aljundi2017, Snell2017, Vinyals2016} and adapt them to Continual Meta-Learning setting.
%
Specifically, MAML~\cite{Finn2017} was used as a baseline, which is a representative optimization-based meta-learner.
%
We only fine-tune the MAML model whenever a new task arrives and call it \textbf{MAML+FT}.
Moreover, for fair comparisons, we also extended MAML to support continual learning by integrating MAS~\cite{Aljundi2018} into its optimization framework, which
is a well-known regularization-based approach proposed particularly for continual learning.
Specifically, we computed the importance for each parameter in the model using the method in MAS,
added them as a regularization term into the loss function and meta-trained the model using MAML's optimization framework.
%
This method is called \textbf{MAML+MAS} in the following.
%
For both MAML+FT and MAML+MAS, since tasks arrive one by one in a sequence (instead of in a batch), we updated the models sequentially using data corresponding
to each incoming task.
%
In addition, Matching Networks~\cite{Vinyals2016} (MN) and Prototypical Networks~\cite{Snell2017} (PN) are both metric-based
few-shot learning
% \Red{few-shot learning}
methods, which were used as baselines too.
Since they do not have the fast-learning phase as MAML and CML, which learns from the $\bD_{train}$ of each arriving task,
they can't be fine-tuned on current task.
%
Again for fair comparisons, during meta-testing, we upgraded both methods as \textbf{MN+CSM} and \textbf{PN+CSM} by integrating our Class Storage Module (CSM) and
storing the class prototypes for each task, 
which helps them
overcome catastrophic forgetting as CML.

%----------------------------------
\begin{figure*}[t]
% \setlength{\abovecaptionskip}{0pt}
\centering
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[scale=0.57]{Figure/MiniImageNet_1shot.png}
% \caption{5-way 1-shot 4 tasks sequence on MiniImageNet}
\caption{Classification accuracies on the timeline of 4 tasks sequence on MiniImageNet (5-way, 1-shot)}
\label{Fig:MiniImageNet_1shot}
\end{figure*}

%----------------------------------
% \begin{figure*}[t]
% \setlength{\abovecaptionskip}{0pt}
% \centering
% %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \includegraphics[scale=0.37]{MiniImageNet_5shot.jpg}
% \caption{5-way 5-shot learning on MiniImageNet}
% \label{Fig:MiniImageNet_5shot}
% \end{figure*}

\begin{figure*}[t]
\centering
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[scale=0.57]{Figure/MiniImageNet_5shot.png}
% \caption{5-way 5-shot 4-tasks sequence on MiniImageNet}
\caption{Classification accuracies on the timeline of 4 tasks sequence on MiniImageNet (5-way, 5-shot)}
\label{Fig:MiniImageNet_5shot}
\end{figure*}
%----------------------------------

\subsection{Experimental Results}
\label{Sec:Results}

%We conducted comprehensive experiments for various possible cases.
%
Tables~\ref{mini-1shot} and~\ref{mini-5shot} show the image classification accuracy (with a confidence interval of $95\%$) given by each method
on each task at the end of the 4-tasks sequence on the MiniImageNet dataset.
%
Tables~\ref{CIFAR-1shot} and~\ref{CIFAR-5shot} show the corresponding results on the CIFAR100 dataset.
%
We can make the following observations from these results.
%
%The Figures~\ref{Fig:MiniImageNet_1shot},~\ref{Fig:MiniImageNet_5shot} show the degree of catastrophic forgetting on each task as each task arrives in a sequence order on MiniImageNet. The X axis represents the order in which the tasks arrive and the Y axis represents the accuracy on each task. We also have result figures on CIFAR100, but we can't display them in paper because of the space limitation of paper.

First of all, CML consistently outperforms all the other methods by relatively large margins
on all the 4 tasks in both 5-way, 1-shot and 5-way, 5-shot cases on both datasets.
%
%For instance, in Table~\ref{mini-1shot}, CML achieves an accuracy of $53.47\%$ on the second task in the 5-way, 1-shot setting, while MAML, MAML-MAS, Matching Networks and %Prototypical Networks only provide $27.84\%$, $27.99\%$, $43.54\%$ and $48.63\%$ accuracies respectively.
%
For instance, from Table~\ref{mini-1shot}, we can see that CML achieves an average accuracy of $58.66\%$,
while the average accuracies given by the other four baselines are
$48.44\%, 43.26\%, 30.31\%. 29.93\%$ respectively. Similar observations can be made from the other three tables.
%
This observation shows that the proposed CML is indeed effective for continual few-shot learning and is superior to
the other meta-learners in terms of classification accuracy.

%\sout{
%Second, the optimization-based meta-learner, MAML, suffers from catastrophic forgetting.
%For instance, from Table~\ref{mini-5shot}, we can observe that at the end of the 4-task sequence,
%MAML offers a reasonable accuracy of $49.34\%$ on task 4, while, it gives fairly low accuracies for
%the previous tasks (i.e., tasks 1, 2, and 3), especially the accuracy on the earliest task (i.e., task 1)
%is only $29.74\%$, which is much lower than that on the most recent task (i.e., task 4).
%}
%
%\sout{
%This is because MAML does not contain a mechanism that is capable of retaining old knowledge.
%Every time when a new task arrives, its model is updated towards a direction that is good for new concepts
%of the new task but may not be favorable for previous tasks.
%}
%
%But why MAML can't achieve high performance even on a new task? Because the training on previous tasks has made MAML model deviated from the good initialization after %meta-training, then MAML model can't adapt to new tasks during \emph{fast-learning} (typically only 5 training steps).

%\sout{It is interesting to see that similar to MAML, MAML-MAS still suffers from catastrophic forgetting.}
%
Second, MAML+FT and MAML+MAS suffer from catastrophic forgetting.
For instance, from Table~\ref{mini-5shot}, we can see that at the end of the 4-tasks sequence,
MAML+MAS provides an accuracy of $50.52\%$ for task $\mathcal{T}_4$, while accuracies on
the previous tasks are pretty low; and the earlier the task, the worse the accuracy.
%
% \Red{Corresponding, the BWT of MAML is $xxx$ and of MAML-MAS is $xxx$.}
%
This observation shows that a regularization-based method is not effective for mitigating the forgetting problem
in the context of few-shot learning.
%
Even though MAML+MAS calculates the importance of each parameter in model
and uses them as a regularization term to penalize the change of model parameters,
the numbers of training samples ($N \times K$) and training steps (typically no more than 5)
are too small to precisely measure the importance of parameters and give proper penalties.
%
Hence, MAS may work well regular continual learning task but turns out to be ineffective for
continual few-shot learning. This also indicates that regularization may not be a right way for
dealing with continual few-shot learning tasks.

In contrast, CML successfully overcomes catastrophic forgetting by consistently maintaining high accuracies on both the most recent task
and the previous tasks. For example, from Table~\ref{mini-5shot}, we can see that CML achieves a high average accuracy
of $70.48\%$, and more importantly, the accuracies on the $4$ tasks are all close to $70\%$.
%
% \Red{At the same time, CML gain a $0.00$ BWT which means it totally avoid the the forgetting problem.}
%
CML delivers such superior performance in this regard because it tackles the forgetting problem with
a rather direct mechanism by storing the class vectors in the memory with a small footprint and retrieving them
when needed.
%
%The key point is that CML stores class vectors $\bV$ of previous tasks in physical memory with only 25KB (3200 float64 data) per class vector $\bV_l$. This memory %consumption is almost negligible under the physical memory capacity of modern computers. And we can continue to reduce memory consumption by reducing the dimension $z$ %(e.g., 3200 in our experiments) of each class vector $\bV_l$.

Third, from these tables, we also notice that MN+CSM and PN+CSM well overcome catastrophic forgetting by maintaining high accuracies for all the previous tasks.
% \Red{with their BWT are both $0.00$}.
These results further show the effectiveness of the memory-based mechanism for continual learning, which has been utilized by CML, MN+CSM and PN+CSM.
%
%\Red{Note that Matching/Prototypical Networks did not utilize this memory-based mechanism in the original paper, and we modified their code here for comparison.}
%
Even though MN+CSM and PN+CSM have the ability to overcome catastrophic forgetting,
%
CML beats them by relatively large margins in terms of classification accuracies, especially on the 1-shot learning tasks. For example, from Table~\ref{mini-1shot},
CML improves the average accuracy from $43.26\%$ and $48.44\%$ to
$58.66\%$.
%
As mentioned above, 
% \Red{we believe that the Teacher Network pre-trained on $\mathscr{D}_{meta-train}$ 
% obtains enough prior knowledge which can guide the Student Network to find a better initialization from which a new task can be more easily solved, though the class labels in $\mathscr{D}_{meta-train}$ and $\mathscr{D}_{meta-test}$ are not overlapping.}
% Besides that, 
CML integrates metric-based classification and adversarial learning
into an optimization-based meta-training framework which, we believe, leads to performance improvements
over the state-of-the-art metric-based methods on these few-shot learning tasks.
%
%From Table~\ref{mini-1shot},~\ref{mini-5shot}, the results indicate that CML can achieve $52.59\%$ average accuracy on 5-way, 1-shot tasks and $68.83\%$ average accuracy on 5-way, 5-shot tasks, while Matching Networks can only achieve $43.26\%$ and $53.92\%$ and Prototypical Networks can achieve $48.44\%$ and $66.45\%$ on 5-way, 1-shot and 5-way, 5-shot tasks respectively.
%We attribute the reasons why CML can achieve the highest accuracies to the following:
%1) We use a pre-trained Teacher Network $F_{\btheta_t}(\cdot)$ which can clearly teach student network which kinds of features to learn;
%2) We use a pre-trained ResNet50~\cite{He2015} as the initial point of Student Network $G_{\btheta_s}(\cdot)$ which already has basic ability to extract features and from where it can absorb knowledge from teacher network more effectively;
%3) We train Student network $G_{\btheta_s}(\cdot)$ in a MAML-similar way. After \textbf{meta-training},  Student network $G_{\btheta_s}(\cdot)$ can get a good initialization from where it can adapt to a new task given a few examples.
%4) We use Discriminator $D_{\btheta_d}(\cdot)$ to learn with Student network $G_{\btheta_s}(\cdot)$ alternately, which makes Student network $G_{\btheta_s}(\cdot)$ generates more discriminative and representative class vectors $\bV$.

% \sout{In addition, as expected, no matter which method is used, the accuracies increase when the number of shots $K$ (i.e., training samples for each task)
% increases from $1$ to $5$. Moreover, there are noticeable improvements on accuracies when moving from MiniImageNet to CIFAR100.
% No matter which dataset is used, CML consistently outperforms all the others.}
%
%For CIFAR100, in Tables~\ref{CIFAR-1shot},~\ref{CIFAR-5shot}, we have similar observations like the results on MiniImageNet.
%In addition, we notice that whether in case of 5-way, 1-shot tasks or 5-way, 5-shot tasks, CML and all other baseline methods, especially Matching Networks, have significantly improvements of classification accuracy on CIFAR100 comparing to MiniImageNet.
%For example, Matching Networks method can achieve classification accuracies of $65.74\%$, $65.80\%$, $64.57\%$ and $66.06\%$ on CIFAR100 for 5-way, 5-shot tasks $\mathcal{T}_1 \dots \mathcal{T}_4$ which are $12.06\%$, $11.69\%$, $10.44\%$ and $12.29\%$ improvements comparing to the results on MiniImageNet.

To better show the change of accuracy during the arriving process of tasks, we plot Figures~\ref{Fig:MiniImageNet_1shot} and ~\ref{Fig:MiniImageNet_5shot}.
%  and~\ref{Fig:MiniImageNet_5shot}.
%and ~\ref{Fig:MiniImageNet_5shot}.
%
In these figures, the x-axis gives the time-step corresponding to the completion of learning for each task and each sub-figure shows the change of accuracy of each task following the timeline. Note that at the time-step of task $\mathcal{T}_j$, we cannot measure the accuracy of task $\mathcal{T}_i (i>j)$, so the corresponding accuracies are simply set to $0$. For example, on the
third sub-figure (corresponding to task $\mathcal{T}_3$) of Figure~\ref{Fig:MiniImageNet_1shot}, we can see that the accuracies corresponding to the time-steps of tasks $\mathcal{T}_1$ and $\mathcal{T}_2$ are set to $0$. From this figure, we can clearly see that CML, MN+CSM and PN+CSM can well overcome catastrophic forgetting. For example, in the first sub-figure of Figure~\ref{Fig:MiniImageNet_1shot}, the curves corresponding to these three algorithms are basically straight horizontal lines, i.e., the
accuracies do not change with the arrival of new tasks.
%
However, both MAML+FT and MAML+MAS suffer from serious forgetting problems. For instance, in the same sub-figure, if MAML+FT is used, the accuracy of task $\mathcal{T}_1$ drops sharply from over $45\%$, which is higher than that given by MN+CSM,
all the way down to $26.85\%$ during the arriving process of all the 4 tasks. 
This observation further shows that MAML is indeed an effective meta-learner for few-shot learning setting 
but behaves poorly on continual learning due to lack of an effective mechanism for retaining old knowledge.
%
%\sout{
%An interesting observation is that the accuracy of a new task given by MAML or MAML-MAS is quite satisfying or even higher than that given by Matching Networks.
%For example, in the first sub-figure of Figures~\ref{Fig:MiniImageNet_1shot}, when task 1 just arrives, the accuracy given by MAML is about $45\%$, which is higher than that
%given by Matching Network. This observation further shows that MAML is indeed an effective meta-learner but behaves poorly on continual learning due to lack of an effective %mechanism for retaining old knowledge.
%}
%
Due to the limited space, we cannot include the figures corresponding to the experimental results on CIFAR100.
but we can see very similar patterns and make similar observations from the Figures~\ref{Fig:MiniImageNet_1shot} and~\ref{Fig:MiniImageNet_5shot}.

\subsection{Ablation Study}
\label{Sec:Study}

We performed an ablation study 
to verify the effectiveness
% for verifying the effectiveness 
of the adversarial training
by comparing CML with the Discriminator and without the Discriminator.
In Table~\ref{AB-study}, we can observe that the Discriminator leads to  $1.75\%$, $0.88\%$, $1.13\%$ and $1.95\%$ improvements in terms of the average accuracy on MiniImageNet and CIFAR100
for 5-way,1-shot and 5-way,5-shot tasks.
As mentioned in Section 4.2, the adversarial training in the meta-update does not have the limitation of few-shot setting due to the relatively more samples for each class.
%
Meanwhile, 
the Teacher Network, through pre-training on $\mathscr{D}_{meta-train}$ with enough samples, can generate a good feature map for each image, which serves as a learning template for the Student Network.
%
Thus, the adversarial training, with the help of the pre-trained Teacher Network, can guide the Student Network to obtain discriminative class vector on unseen categories and
achieve a better initialization, from where the tasks, each with a few samples, can be easily handled.

% \Red{
%Since the Teacher Network pre-trained on the $\mathscr{D}_{meta-train}$ including enough samples can generate good feature maps serving as learning templates for the Student Network, 
% with the adversarial training introduced in the meta-update rather than the fast-learning, which gets rid of the limitation of few-shot setting, 
% the Discriminator boosts the Student Network to absorb more knowledge from the Teacher Network and arrive at a better initialization from where new tasks with a few samples can be handled more easily.}
%
% \Red{Since the Teacher Network is pre-trained on the $\mathscr{D}_{meta-train}$ including enough samples which provide considerable prior knowledge,} 
% % \sout{Since the Discriminator regards features extracted from the Teacher Network as true samples and class vectors from the Student Network as false samples,}
% % \sout{it promotes a feature alignment between the Teacher Network and the Student Network, which boosts the Student Network to absorb more knowledge from the Teacher Network.}
% \Red{the adversarial training promotes a feature alignment between the Teacher Network and the Student Network, which boosts the Student Network to absorb more knowledge from the Teacher Network and arrive at a better initialization from where new tasks with a few samples can be handled more easily.}
%
%And the teacher network has achieved a good enough performance on the categories in meta-set $\mathscr{D}_{meta-train}$, which is beneficial to student network to gain more %discriminative features on unseen categories.


% \begin{figure*}[t]
% \centering
% %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \includegraphics[scale=0.35]{CIFAR100_1shot.png}
% \caption{5-way 1-shot learning on CIFAR100}
% \label{Fig:CIFAR100_1shot}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \includegraphics[scale=0.35]{CIFAR100_5shot.png}
% \caption{5-way 5-shot learning on CIFAR100}
% \label{Fig:CIFAR100_5shot}
% \end{figure*} 

==> Continual Few-Shot Learning_Arxiv/6-Conclusions.tex <==
%-----------------------------------------------------------------
\begin{table}[t]\scriptsize
\centering
\caption{Average accuracies given by CML with (w.) and without (wo) the Discriminator.}
\renewcommand\arraystretch{1.3}
\begin{tabular}{|c|c|c|c|c|}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{|c|}{MiniImageNet} & \multicolumn{2}{|c|}{CIFAR100} \\
 & 5-way,1-shot & 5-way,5-shot & 5-way,1-shot & 5-way,5-shot\\ \midrule
CML wo D & $56.91\%$ & $69.6\%$ & $60.95\%$ & $72.08\%$ \\ 
CML w. D& \bm{$58.66\%$} & \bm{$70.48\%$} & \bm{$62.08\%$} & \bm{$74.03\%$} \\ \bottomrule
% CML(Ours) & \sout{\bm{$71.57\pm1.59\%$}} & \sout{\bm{$70.10\pm1.68\%$}} & \sout{\bm{$70.86\pm1.64\%$}} & \sout{\bm{$71.08\pm1.65\%$}} & \sout{\bm{$70.09\%$}} \\ \hline

\end{tabular}
\label{AB-study}
\end{table}
%-----------------------------------------------------------------

\section{Conclusions}
\label{Sec:Conclusions}

In this paper, we studied a new problem called continual few-shot learning,
in which a sequence of tasks arrives one by one, each of which only contains a few training samples.
%
We proposed a novel model-agnostic meta-learner, Continual Meta-Learner (CML), which
integrates metric-based classification and a memory-based mechanism along with adversarial
learning into an optimization-based meta-learning framework.
%
It has been shown by extensive experimental results on MiniImageNet and CIFAR100
that CML consistently outperforms the four baselines in terms of classification accuracy by large margins
in both the 5-way,1-shot and 5-way,5-shot cases, and successfully overcomes catastrophic forgetting; while
the optimization-based meta-learner suffers from severe forgetfulness.



==> Continual Few-Shot Learning_Arxiv/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Continual Few-Shot Learning_Arxiv/macro.tex <==
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{epsfig}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{multirow}
\usepackage{color}
\usepackage[normalem]{ulem}
% \usepackage{caption} 
\usepackage{booktabs}
% \captionsetup[table]{skip=5pt}


\newcommand{\Red}        {\textcolor{red}}
\newcommand{\Yel}        {\textcolor{yellow}}
\newcommand{\Blue}        {\textcolor{blue}}

\newcommand{\kETAL}     {\textit{et al.}}
\newcommand{\bx}        {\textbf{x}}
\newcommand{\by}        {\textbf{y}}
\newcommand{\bD}        {\textbf{D}}
\newcommand{\bV}        {\textbf{V}}
\newcommand{\bX}        {\textbf{X}}
\newcommand{\bY}        {\textbf{Y}}
\newcommand{\bM}        {\textbf{M}}
\newcommand{\mD}        {\mathcal{D}}
\newcommand{\btheta}    {\bm{\theta}}
\newcommand{\mT}        {\mathcal{T}}
\newcommand{\mL}        {\mathcal{L}}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

